Search for New Physics in Lepton + Photon + X Events with 929 pb-1 of ppbar Collisions at roots = 1.96 TeV

We present results of a search at CDF in 929 pb-1 of ppbar collisions at 1.96 TeV for the anomalous production of events containing a high-transverse momentum charged lepton (either electron or muon) and photon, accompanied by missing transverse energy (MET), and/or additional leptons and photons, and jets (X). We use the same selection criteria as in a previous CDF Run I search, but with an order-magnitude larger data set, a higher ppbar collision energy, and the CDF II detector. We find 163 Lepton + Photon + MET + X events, compared to an expectation of 150.6+-13.0 events. We observe 74 Multi-Lepton + Photon + X events, compared to an expectation of 65.1+-7.7 events. We find no events similar to the Run I 2 electrons + 2 photons + MET event.

==> flow_chart_landscape.tex <==
\begin{figure}[!b]
\thicklines
\begin{center}
\framebox(135,50)[s]{
{
\begin{minipage}{135pt}
\begin{center}
$\lgX$ Sample \\
%1 Lepton and 1 Photon \\
$\Etgamma\gt 25$ GeV, $\Etlepton\gt 25$ GeV \\
{\bf\noflg (\nofmug~and~\nofeg)} \\
%Events
\end{center}
\end{minipage}
}
}
\put(-10,0){\vector(0,-1){10}}
\put(-125,0){\vector(0,-1){10}}
%\vspace{-1pt}

\framebox(115,50)[0,0] {
{
\begin{minipage}{115pt}
\begin{center}
Exactly 1 $\ell$, 1 $\gamma$ \\
$\Delta\phi_{l\gamma}\gt 150^\circ$, $\met\lt 25~\GeV$ \\
{\bf\noflgdphi(\nofmugdphi~and~\nofegdphi)} \\
%Events
\end{center}
\end{minipage}
}
}
\put(-60,0){\vector(0,-1){8}}
\put(-115,0){\vector(0,-1){70}}
\makebox(10,30)[l]{}
\framebox(115,50)[0,0]{
{
\begin{minipage}{115pt}
\begin{center}
Inclusive \\
Multi-Body $\lgX$ \\
{\bf\noflgallother(\nofmugallother~and~\nofegallother)} \\
%Events
\end{center}
\end{minipage}
}
}
\put(0,0){\vector(0,-1){70}}
\put(-115,0){\vector(0,-1){70}}
\put(-60,0){\vector(0,-1){8}}
\end{center}

\vspace{-123pt}

%Landscape
\makebox(243,50)[l]{}
%Portrait
%\makebox(100,60)[l]{}
\framebox(110,50)[0,0]{
{
\begin{minipage}{110pt}
\begin{center}
Z-Like $\lgal$ \\
$81~\GeV<M_{e\gamma}<101~\GeV$\\
%(Background Calibration) \\
{\bf\noflgzlike(\nofmugzlike~and~\nofegzlike)} \\
%Events
\end{center}
\end{minipage}
}
}
\makebox(12,50)[l]{}
\framebox(110,50)[0,0]{
{
\begin{minipage}{110pt}
\begin{center}
Exactly 1 $\ell$, 1 $\gamma$, \\
$\Delta\phi_{l\gamma}<150^\circ$, $\met<25~\GeV$ \\
{\bf\noflgzunlike(\nofmugzunlike~and~\nofegzunlike)} \\
%Events
\end{center}
\end{minipage}
}
}

\begin{center}
\framebox(80,50)[0,0]{
{
\begin{minipage}{80pt}
\begin{center}
Two-Body Events \\
{\bf \noflgtwobody(\nofmugtwobody~and~\nofegtwobody)} \\
%Events
\end{center}
\end{minipage}
}
}
\framebox(80,50)[0,0]{
{
%\color{red}\bf
\begin{minipage}{80pt}
\begin{center}
$\lgmet$, \\
$\met> 25~\GeV$\\
{\color{black}\bf \noflglgmet(\nofmuglgmet~and~\nofeglgmet)} \\
%Events
\end{center}
\end{minipage}
}
}
\framebox(80,50)[0,0]{
{
%\color{red}\bf
\begin{minipage}{80pt}
\begin{center}
$\llg$ Events \\
{\color{black}\bf\noflgmultil(\nofmugmultil~and~\nofegmultil)}\\
$\lgg$ Events \\
{\color{black}\bf none observed}
%{\color{black}\bf\noflgmultig(\nofmugmultig~and~\nofegmultig)}
\end{center}
\end{minipage}
}
}
\end{center}
%\end{document}\caption{Muon Control Sample}
\caption{$\lgX$ Sample: the subsets of inclusive lepton-photon events analyzed. The number of events in each subcategory is given as a sum of muons and electrons. The first term in parethesis refers to $\mugX$ while the latter refers to the $\egX$.}
\label{flowchart_lepton.figure}
\end{figure}

